Intrinsic nonlinear elasticity: An exterior calculus formulation

In this paper we formulate the theory of nonlinear elasticity in a geometrically intrinsic manner using exterior calculus and bundle-valued differential forms. We represent kinematics variables, such as velocity and rate-of-strain, as intensive vector-valued forms while kinetics variables, such as stress and momentum, as extensive covector-valued pseudo-forms. We treat the spatial, material and convective representations of the motion and show how to geometrically convert from one representation to the other. Furthermore, we show the equivalence of our exterior calculus formulation to standard formulations in the literature based on tensor calculus. In addition, we highlight two types of structures underlying the theory. First, the principle bundle structure relating the space of embeddings to the space of Riemannian metrics on the body, and how the latter represents an intrinsic space of deformations. Second, the de Rham complex structure relating the spaces of bundle-valued forms to each other.

==> internal_discussions.tex <==

\begin{discussion}\label{disc:Stefano1}
	\stefano{IT MAY BE THE CASE BUT WHY ? THERE SHOULD BE CLEAR PHYSICAL REASONS WHY THAT IS NEEDED CONSIDERING THE BODY ABSTRACTION IS LIVING IN A AMBIENT SPACE WHICH HAS A VOLUME}\\
	\fede{The construction is clear and standard, but I would like to ask you an opinion: the fact that $\cl{B}$ is equipped with a volume form implies that $\int_{\cl{B}} \vFB$ exists and is well defined. Clearly it is not representing the physical "volume" of the object, since it depends of the metric (e.g., expansion along the deformation)..does the integral have an interpretation? (in my opinion it does not.)}
\end{discussion}

\begin{discussion}\label{disc:Fede2}
	\fede{difference between tangent map and pushforward? I guess $T\cfgInvT(x,v)=(\cfgInvT(x),\cfgInvT^*v)$, i.e. pushforward is only the second slot of the tangent map}
	\ramy{Yes, that's terminology. Some references call both the tangent map and its action on tensor fields by the pushforward (I think Frederic did that in his course)}
\end{discussion}

\begin{discussion}\label{disc:Fede1}
	\fede{I think an useful notation, which will come useful when discussing the dualities, is the one we used for the moving domain paper: $\vM_t \in \spVecS \otimes_{\cfgT} \Omega^0(B)$, which is another way to say $\spVecPhi$ (right?) but it immediately makes clear the nature of two-point tensor, which the material velocity is, with distinction first-second leg..in this view "true" vector fields are vector valued zero-forms, and "false" ones are two point tensors of the same valence but the the legs on different manifolds.}
	
	\fede{As before, I think the two-point tensor notation $F \in \spVec{S} \otimes_{\cfgT} \Omega^1(B)$ and $F^{-1} \in \spVec{B} \otimes_{\cfgInvT} \Omega^1(S)$ are helpful, because the notation tells you immediately how the dual element should be...but maybe I am biased..}
\end{discussion}


\begin{discussion}\label{disc:Andrea1}
	\andrea{The coordinate expression of the vector fields should be also maps from euclidean to euclidian. The maps you represent here are ($P \in \cl{U} \subset \cl{B}, \; Q \in \cl{V} \subset \cl{S}$)
		\begin{equation}
			\begin{aligned}
				&\map{\vS^i(Q, t) = \tilde{\mathbf{v}}^i \circ \bm{X} \circ \cfgInvT}{\cl{V} \times [0, T]}{\bb{R}},\\
				&\map{\vC^I(P, t) = ((\Finvr)^I_i \circ \bm{x} \circ \cfgT) \left(\bm{x} \circ \frac{\partial \phi_t}{\partial t}\right)}{\cl{U} \times [0, T]}{\bb{R}},
			\end{aligned}
		\end{equation}
		If one wants a coordinates representation of these two variables associated to the corresponding bases it should be
		\begin{equation}
			\begin{aligned}
				&\map{\mathbf{v}^i(\bm{x}, t) = \tilde{\mathbf{v}}^i \circ \bm{X} \circ \cfgInvT \circ \bm{x}^{-1} = \tilde{\mathbf{v}}^i \circ \bm{\phi}_t^{-1}(\bm{x})}{\bb{R}^3 \times [0, T]}{\bb{R}},\\
				&\map{\hat{\mathbf{v}}^I(\bm{X}, t) = ((\Finvr)^I_i \circ \bm{x} \circ \cfgT \circ \bm{X}^{-1}) \left(\bm{x} \circ \frac{\partial \phi_t}{\partial t} \circ \bm{X}^{-1}\right)}{\bb{R}^3 \times [0, T]}{\bb{R}}, \\
				&\qquad= ((\Finvr)^I_i \circ \bm{\phi}_t(\bm{X})) \tilde{\mathbf{v}}^i(\bm{X}, t)
			\end{aligned}
		\end{equation}
	}
\end{discussion}

\begin{discussion}\label{disc:Andrea2}
	\andrea{If $\cl{S}$ is supposed to be a Riemmanian manifold then one needs to consier covariant differentiation for the material velocity, i.e.
		\begin{equation*}
			\tilde{a}_t = \partial_t \vM_t = \frac{D \vM_t}{\partial t}.
		\end{equation*}
		In coordinates
		\begin{equation*}
			\tilde{a}_t^i =\frac{\partial^2 \phi_t^i}{\partial^2 t} + (\Gamma_{jk}^i \circ \phi_t) \frac{\partial \phi_t^j}{\partial t} \frac{\partial \phi_t^k}{\partial t}
		\end{equation*}
	}
	
	\ramy{I don't see why !} \andrea{Me neither but this is presented by Yavari in his papers.}
\end{discussion}

\begin{discussion}\label{disc:Andrea3}
	\andrea{The coordinate definition of $\cfgT^i$ should be $\map{\bm{\phi}_t = \phi_{t, I}^i:= \B{x}\circ \cfgT \circ \B{X}^{-1}}{\bb{R}^3 \times [0, T]}{\bb{R}^3}$, otherwise the Jacobian $F^i_I = \frac{\partial \cfgT^i}{\partial X^I}$ cannot be computed. Similarly for $(\Finvr)^I_i = \frac{\partial (\cfgInvT)^I}{\partial x^i}$. Consequently for the velocity coordinates $ \map{\tilde{\mathbf{v}}^i(\bm{X}, t):= \frac{\partial \bm{\phi}_t^i}{\partial t}(\bm{X})}{\bb{R}^3 \times [0, T]}{\bb{R}}.$ }
	
	\ramy{I checked with several references e.g. Yavari's 2006 paper, and I found that they write it like that. Maybe they suppress this technical details. I'm not sure ! }
\end{discussion}
